Cohomology in Constraint Satisfaction and Structure Isomorphism

Constraint satisfaction (CSP) and structure isomorphism (SI) are among the most well-studied computational problems in Computer Science. While neither problem is thought to be in $\texttt{PTIME},$ much work is done on $\texttt{PTIME}$ approximations to both problems. Two such historically important approximations are the $k$-consistency algorithm for CSP and the $k$-Weisfeiler-Leman algorithm for SI, both of which are based on propagating local partial solutions. The limitations of these algorithms are well-known; $k$-consistency can solve precisely those CSPs of bounded width and $k$-Weisfeiler-Leman can only distinguish structures which differ on properties definable in $C^k$. In this paper, we introduce a novel sheaf-theoretic approach to CSP and SI and their approximations. We show that both problems can be viewed as deciding the existence of global sections of presheaves, $\mathcal{H}_k(A,B)$ and $\mathcal{I}_k(A,B)$ and that the success of the $k$-consistency and $k$-Weisfeiler-Leman algorithms correspond to the existence of certain efficiently computable subpresheaves of these. Furthermore, building on work of Abramsky and others in quantum foundations, we show how to use \v{C}ech cohomology in $\mathcal{H}_k(A,B)$ and $\mathcal{I}_k(A,B)$ to detect obstructions to the existence of the desired global sections and derive new efficient cohomological algorithms extending $k$-consistency and $k$-Weisfeiler-Leman. We show that cohomological $k$-consistency can solve systems of equations over all finite rings and that cohomological Weisfeiler-Leman can distinguish positive and negative instances of the Cai-F\"urer-Immerman property over several important classes of structures.

==> algorithm.tex <==
%TODO:
%-incorporate handwritten notes

In this section, we define the cohomological $k$-consistency algorithm and
the relation $\rightarrow^{\mathbb{Z}}_k$ that it computes between
structures. We also show that the algorithm runs in polynomial
time in the product of the sizes of the input structures and that
the relation is compositional.


\subsection{Classical $k$-consistency algorithm}
We start by recalling some definitions related to the
classical $k$-consistency algorithm on which our algorithm will build.


For $A$ and $B$ finite structures over a common (finite) signature,
let $\mathbf{Hom}_k(A, B)$ denote the set of partial homomorphisms
from $A$ to $B$ with domain of size less than or equal to $k$. There
is a natural partial order $<$ on this set, defined
as follows.  For any partial homomorphisms $f,g \in \mathbf{Hom}_k(A, B)$
we say that $f < g$ if $\mathbf{dom}(f) \subset \mathbf{dom}(g)$
and $g_{\mid_{\mathbf{dom}(f)}} = f$.

We say that any $S \subset \mathbf{Hom}_k(A,B)$ has the \emph{forth}
property if for every $f \in S$ with $|\mathbf{dom}(f)|< k$
we have the property $\mathbf{Forth}(S,f)$ which is defined as follows:
$$  \ \forall a \in A, \
        \exists b \in B \text{ s.t. } f \cup \{(a,b)\} \in S. $$

Given $S \subset \mathbf{Hom}_k(A,B)$ we define $\overline{S}$ to
be the largest subset of $S$ which is downwards-closed and has the
forth property. Note that $\emptyset$ satisfies these conditions,
so such a set always exists. For a fixed $k$ there is a simple
algorithm for computing $\overline{S}$ from $S$.

This is done by starting with $S_0 = S$ and then entering the
following loop with $i=0$
\begin{enumerate}
  \item Initialise $S_{i+1}$ as being equal to $S_i$.
  \item For each $s \in S_{i}$, check if $\mathbf{Forth}(S_i,s)$ holds and
  if not remove it from $S_{i+1}$ along with all $s'> s$.
  \item If none fail this test, halt and output $S_i$.
  \item Otherwise, increment $i$ by one and repeat.
\end{enumerate}
It is easily seen that this runs in polynomial time in $\abs{A}\abs{B}$.

%this subsection is in progress and needs work from here down.
Now for a pair of structures $A, B$ we say that the pair
$(A,B)$ is $k$ consistent if $\overline{\mathbf{Hom}_k(A,B)} \neq \emptyset$.
We denote this by writing $A \rightarrow_k B$ and the algorithm above
shows how to decide this relation in polynomial time for fixed $k$.
This relation has many equivalent logical and algorithmic definitions
as seen in \cite{federvardi}, and \cite{BartoKozik}.


\subsection{Local, global \& $\mathbb{Z}$-linear sections}

Let $S$ be some set $\emptyset \neq S \subset \mathbf{Hom}_k(A,B)$.
Let $A^{\leq k}$ be the set of all subsets of $A$ with at most $k$
elements and for each $\mathbf{a} \in A^{\leq k}$ we consider the
\emph{set of local sections of $S$ at $\mathbf{a}$ }
$$ S_{\mathbf{a}} = \{ f \in S \ \mid \ \mathbf{dom}(f) = \mathbf{a} \} $$

Given such a section $s \in S_{\mathbf{a}}$, it is natural to ask whether it
can be extended to a homomorphism $f: A \rightarrow B$ such that
$f_{\mid_\mathbf{a}} = s$. If we ask that $f$ should locally look like a section
of $S$ at every $\mathbf{a}' \in A^{\leq k}$ then the existence of such an
$f$ is equivalent to the existence of a set $\{ s_{\mathbf{a}'} \in S_{\mathbf{a}'} \}_{\mathbf{a}' \in A^{\leq k}}$
such that $s_\mathbf{a} = s$ and for all $\mathbf{a}_1, \mathbf{a}_2 \in A^{\leq k}$ the
corresponding local sections agree on the intersection $\mathbf{a}_1 \cap \mathbf{a}_2 $, i.e.\
$$s_{\mathbf{a}_1\mid_{\mathbf{a}_1\cap\mathbf{a}_2}} = s_{\mathbf{a}_2\mid_{\mathbf{a}_1\cap\mathbf{a}_2}}.$$
We call such a set a \emph{global section of $S$ extending $s$} and
if one exists we say that $s$ is \emph{extendable in $S$}.
Deciding whether there is such a global section for general $S$ is
equivalent to deciding $\mathbf{CSP}$ and is, thus, \texttt{NP-Complete}.
In our algorithm we will ask for the following weaker but efficiently computable
relaxation of this condition.

Let $\mathbb{Z}S_{\mathbf{a}}$ be the formal $\mathbb{Z}$-linear
combinations of elements of $S_{\mathbf{a}}$. We call these \emph{local
$\mathbb{Z}$-linear sections at $\mathbf{a}$}. For any $\mathbf{a}'
\subset \mathbf{a}$ and any local $\mathbb{Z}$-linear section $r = \sum_{s\in S_{\mathbf{a}}}z_s s
\in \mathbb{Z}S_{\mathbf{a}}$, we write $r_{\mid_{\mathbf{a}'}}$
for the restriction of this section to $\mathbf{a}'$ given by
$\sum_{s\in S_{\mathbf{a}}}z_s s_{\mid_{\mathbf{a}'}} \in \mathbb{Z}S_{\mathbf{a}'}$.
We say that $s \in S_{\mathbf{a}}$ is \emph{$\mathbb{Z}$-extendable in $S$}
if there is a global $\mathbb{Z}$-linear section $\{r_{\mathbf{a}'} \in
\mathbb{Z}S_{\mathbf{a}'} \}_{\mathbf{a}' \in A^{\leq k}}$ extending
$s$. By analogy to the case in the previous paragraph we require
that $r_{\mathbf{a}} = s$ and for all $\mathbf{a}_1, \mathbf{a}_2
\in A^{\leq k}$ we have
$$r_{\mathbf{a}_1\mid_{\mathbf{a}_1\cap\mathbf{a}_2}}
= r_{\mathbf{a}_2\mid_{\mathbf{a}_1\cap\mathbf{a}_2}}.$$

We note that a local section $s$ being $\mathbb{Z}$-extendable in a set $S$
implies that $s$ has the forth property and that all $s' < s$ are
contained in $S$

\begin{lem}\label{lem:z_ext}
  For any structures $A$, $B$, positive integer $k$, set $S \subset \mathbf{Hom}_k(A,B)$,
  and local section $s \in S$, if $s$ is $\mathbb{Z}$-extendable in
  $S$ then for all local sections $s' < s$
  $s' \in S$ and, if $|\mathbf{dom}(s)| < k$ then $\mathbf{Forth}(S,s)$ holds.

\end{lem}

\begin{proof}
  Let $\{ r_{\mathbf{a}} = \sum \alpha_f f\}$ be the global $\mathbb{Z}$-linear
  section extending $s$. Now suppose that $s' < s$, i.e.\ that
  there is a $\mathbf{b} \subset \mathbf{dom(s)}$ such that $s' = s_{\mid_{\mathbf{b}}}$.
  However we know that $r_{\mathbf{b}} = (r_{\mathbf{dom}(s)})_{\mid_{\mathbf{b}}}$ and
  as $r$ extends $s$ we have that $r_{\mathbf{dom}(s)} = s$ and so $r_{\mathbf{b}} = s_{\mid_{\mathbf{b}}} = s'$.
  So $s'$ must appear in $r$ and thus appears in $S$. \\
  To show that $\mathbf{Forth}(S,s)$ holds, we consider any $a \in A$
  and we look for a $b \in B$ such that $s \cup \{(a,b) \} \in S$.
  For any such $a$, as $r$ is a
  global $\mathbb{Z}$-linear section, we have that
  $$ (r_{\mathbf{dom}(s) \cup \{a\}})_{\mid_{\mathbf{dom}(s)}} = r_{\mathbf{dom}(s)} = s$$
   However, the coefficients of $s$ in the left hand side, is simply the
   sum of the coefficients of those $s' \in S$ with domain $\mathbf{dom}(s) \cup \{a\}$
   such that $s'_{\mid_{\mathbf{dom}(s)}} = s$. $\mathbf{Forth}(S,s)$ holds
   precisely when such an $s'$ exists for each $a \in A$.
   As the coefficient of $s$ on the right hand side of the equation above is
   always non-zero there must be at least one such $s'$ for each $a$.
\end{proof}

Finally, the conditions defining the $\mathbb{Z}$-extendability of
$s$ in some $S$ are simply systems of $\mathbb{Z}$-linear equations in
the variables $z_s$. Indeed each equality over $\mathbb{Z}S_{\mathbf{a}'}$ in the
definition of $\mathbb{Z}$-extendability yields
at most $|B|^k$ $\mathbb{Z}$-linear equations, one for the coefficient of
each element $s' \in S_{\mathbf{a}'}$.
This means that for any $s \in S$, deciding whether $s$ is $\mathbb{Z}$-extendable
in $S$ is equivalent to deciding if a system of at most $|A|^{2k}\cdot|B|^k$
$\mathbb{Z}$-linear equations, one equation in $\mathbb{Z}S_{\mathbf{a}\cap\mathbf{a}'}$
for each pair $\mathbf{a}, \mathbf{a}' \in A^{\leq k}$, in at most $|A|^{k}\cdot|B|^k$ variablesis solvable over $\mathbb{Z}$.
As such systems of linear equations over $\mathbb{Z}$ can be sovled in
polynomial time in the number of equations and variables via
computing Smith Normal Forms of integer matrices as done by Kannan and Bachem \cite{KannanBachem}),
we can, for fixed $k$, decide whether $s$ is $\mathbb{Z}$-extendable in
$S\subset \mathbf{Hom}_k(A,B)$ in polynomial time in $|A|\cdot|B|$.
Furthermore, we know that if $s$ is extendable then trivially it is $\mathbb{Z}$-extendable.
So removing local sections which fail to be $\mathbb{Z}$-extendable
will not remove any genuine global sections in $S$. This inspires the following algorithm.

\subsection{The cohomological $k$-consistency algorithm}

Here, we describe an extension to the $k$-consistency algorithm which
utilises the notion of $\mathbb{Z}$-extendability.

Take as input a pair of $\sigma$-structures $(A,B)$. Begin by setting
$S_0 = \overline{\mathbf{Hom}_k(A,B)}$
as in the $k$-consistency algorithm then enter the following loop with $i=0$:
\begin{enumerate}
  \item Compute $S_{i+1} = \{s \in S_i \ \mid \ s \text{ is $\mathbb{Z}$-extendable in }S_i \}$
  \item If $S_{i+1} = \emptyset$, then reject $(A,B)$ and halt
  \item If $S_{i+1} = S_i$ then accept $(A,B)$ and halt.
  \item Otherwise, return to Step 1 with $i = i+1$.
\end{enumerate}
 If this algorithm accepts a pair $(A,B)$ we say that $\mathbf{CSP}(A,B)$ is
 cohomologically $k$-consistent and we write $A \rightarrow^{\mathbb{Z}}_k B$.
 It is clear that every element of the set $S$ remaining when this
 algorithm terminates is $\mathbb{Z}$-extendable in $S$. By Lemma \ref{lem:z_ext}, $S$ is
 also downward-closed and has the forth property. Furthermore,
  as $\mathbb{Z}$-extendability in any subset of $S$ implies $\mathbb{Z}$-extendability
  in $S$ (simply by setting any extra coefficients to $0$), we have the following
  observation
  \begin{obs}\label{obs:consist_set}
    For any structures $A$ and $B$ $A \rightarrow^{\mathbb{Z}}_k B$
    if and only if there exists a set $\emptyset \neq S \subset \mathbf{Hom}_k(A,B)$
   in which each element $s \in S$ is $\mathbb{Z}$-extendable in $S$.
  \end{obs}

We now demonstrate some basic facts about this relation and the
given algorithm. Firstly, we show that the algorithm given above is efficient.

\begin{prop}
  For fixed $k$ and fixed finite signature $\sigma$, the relation
  $A \rightarrow^{\mathbb{Z}}_k B$ is decidable in polynomial time in the product of the sizes
  of $A$ and $B$.
\end{prop}
\begin{proof}
We begin by noting that the main loop of the $\rightarrow^{\mathbb{Z}}_k$ algorithm
either results in some $S_{i+1}$ which is strictly smaller than $S_i$ or it halts.
This means that the number of iterations is bounded above by $|S_0|$ which is at
most $|A|^k\cdot|B|^k$, i.e. polynomial in the product of the sizes of $A$ and $B$.

Next we show that each iteration of the loop only takes polynomial time in $|A|\cdot |B|$.
The body of each loop involves deciding, for each $s \in S_i$, whether or not $s$ is
$\mathbb{Z}$-extendable in $S_i$. For each $s$, this means checking the solvability of a system of at most $|A|^{2k}\cdot |B|^k$
$\mathbb{Z}$-linear equations in at most $|A|^{k}\cdot|B|^{k}$ variables, as noted above. This can
be done in polynomial time for each $s$ by the algorithm of Kannan and Bachem \cite{KannanBachem}
and as $|S_i|$ is bounded by $|A|^k\cdot|B|^k$ this whole step takes only polynomial
time in $|A|\cdot |B|$.

As the algorithm terminates if either the loop ends with $S_{i+1} = \emptyset$ or
$S_{i+1} = S_i$ we know that it terminates and combining the arguments of the
previous two paraghraphs we know that it does so in polynomial time in $|A|\cdot |B|$.
\end{proof}

We conclude this section by showing that the relation $\rightarrow^{\mathbb{Z}}_k$ is transitive.
In particular, we prove the following theorem.

\begin{prop}\label{prop:comp}
  For all $k$, given $A, B$ and $ C$ structures over a common finite signature
  $$ A \rightarrow^{\mathbb{Z}}_k B \rightarrow^{\mathbb{Z}}_k C
  \implies A \rightarrow^{\mathbb{Z}}_k C. $$
\end{prop}

\begin{proof}
  Success of the $\rightarrow^{\mathbb{Z}}_k$ algorithm for the pairs $(A,B)$
  and $(B, C)$ results in two non-empty sets $S^{AB} \subset \mathbf{Hom}_k(A,B)$
  and $S^{BC} \subset \mathbf{Hom}_k(B, C)$ in both of which each local section is
  $\mathbb{Z}$-extendable. By Observation \ref{obs:consist_set}, to show that $A \rightarrow^{\mathbb{Z}}_k C$,
  it suffices to show that the set $S^{AC} =
  \{ s \circ t \ \mid \ s \in S^{BC}, t \in S^{AB} \}$ has the same property. \\

\iffalse
\paragraph{Downward-closure}
 Let $p = (s\circ t) \in S^{AC}$. Any $p' < p$ in the partial order
 on $\mathbf{Hom}_k(A,C)$ is given by $p' = p_{\mid_{\mathbf{a}}}$
 for some $\mathbf{a} \subset \mathbf{dom}(p)$. However it is easy to
 see this is the same function as $$ (s_{\mid_{t(\mathbf{a})}} \circ t_{\mid_{\mathbf{a}}}).$$
 As $S^{AB}$ and $S^{BC}$ are downward-closed, these restricted functions
 are in $S^{AB}$ and $S^{BC}$ respectively and so $p' \in S^{AC}$.

\paragraph{Forth property}
  To show that $S^{AC}$ has the forth property we take any $p =  s \circ t \in S^{AC}$
  with $|\mathbf{dom}(p)| = |\mathbf{dom}(t)| < k$ and any
  $a \in A \setminus \mathbf{dom}(p)$. By the forth property of $S^{AB}$,  there
  exists $b \in B$ such that $t \cup \{(a,b)\} \in S^{AB}$. If $b \in \mathbf{dom}(s)$
  then $(s \circ t) \cup \{ (a, s(b)) \} =  s \circ (t\cup \{(a,b)\}) \in S^{AC}$.
  Otherwise, we use the forth property of $S^{BC}$ to find $c \in C$ such that
  $s \cup \{ (b,c) \} \in S^{BC}$ and then
  $(s \circ t) \cup \{ (a, c) \} =  (s \cup \{ (b,c) \}) \circ (t\cup \{(a,b)\}) \in S^{AC}$.\\


\paragraph{$\mathbb{Z}$-extendability property}
\fi

  To show that every $p_0 =  s_0 \circ t_0 \in S^{AC}_{\mathbf{a}_0}$ is $\mathbb{Z}$-extendable in $S^{AC}$ we
  construct a global $\mathbb{Z}$-linear section extending $p_0$ from the
  $\mathbb{Z}$-linear sections $\{r^{t_0}_{\mathbf{a}} := \sum_t z_t t \}_{\mathbf{a}\in A^{\leq k}}$
  and $\{r^{s_0}_{\mathbf{b}} := \sum_s w_s s \}_{\mathbf{b}\in B^{\leq k}}$ extending $t_0$ and $s_0$ respectively.
  Define $\{ r^{p_0}_{\mathbf{a}} \}_{\mathbf{a} \in A^{\leq k}}$ as
  $$ r^{p_0}_{\mathbf{a}} = \sum_{t \in S^{AB}_\mathbf{a}} \sum_{s \in S^{BC}_{t(\mathbf{a})}} z_t w_s (s \circ t)  $$
  To show that this is a global $\mathbb{Z}$-linear section extending
  $p_0$ we need to show firstly that $r^{p_0}_{\mathbf{a}_0} = p_0$
  and secondly that the local sections of $r^{p_0}$ agree on the pairwise
  intersections of their domains.

  To show that $r^{p_0}_{\mathbf{a}_0} = p_0$ we observe that, as
  $r^{t_0}$ $\mathbb{Z}$-linearly extends $t_0$, for all $t \in S^{AB}_{\mathbf{a}_0}$ we have
  \[ z_t = \begin{cases}
        1, & \text{for } t = t_0\\
        0, & \text{otherwise,}
          \end{cases} \]
  and similarly, for all $s \in S^{BC}_{t_0(\mathbf{a}_0)}$
  \[ w_s = \begin{cases}
        1, & \text{for } w = w_0\\
        0, & \text{otherwise.}
          \end{cases} \]
  From this we have that
  $$ r^{p_0}_{\mathbf{a}_0} = z_{t_0} w_{s_0} (s_0 \circ t_0) = p_0 $$
  as required.

  Finally, we need to show for any $\mathbf{a}, \mathbf{a}^{\prime}$ in $A^{\leq k}$
  with intersection $\mathbf{a}^{\prime\prime}$ that
  $$r^{p_0}_{\mathbf{a}\mid_{\mathbf{a}^{\prime\prime}}} = r^{p_0}_{\mathbf{a}^{\prime}\mid_{\mathbf{a}^{\prime\prime}}}.$$
  To do this we show that the left hand side depends only
  on $\mathbf{a}^{\prime\prime}$ and not on $\mathbf{a}$. As this argument
  applies equally to the right hand side, the result follows.

  To begin with the left hand side is a dependent sum which loops over $t \in S^{AB}_{\mathbf{a}}$ and
  $s \in S^{BC}_{t(\mathbf{a})}$  as follows:
  \[
    r^{p_0}_{\mathbf{a}\mid_{\mathbf{a}^{\prime\prime}}} = \sum_{t, s} w_s z_t (s\circ t)_{\mid_{\mathbf{a}^{\prime\prime}}}
  \]
  To emphasise the dependence on $\mathbf{a}^{\prime\prime}$ we
  can group this sum together by pairs $t^{\prime\prime}, s^{\prime\prime}$
  with $t^{\prime\prime} \in S^{AB}_{\mathbf{a}^{\prime\prime}}$
  and $s^{\prime\prime} \in S^{BC}_{t^{\prime\prime}(\mathbf{a}^{\prime\prime})}$.
  Within each group the the sum loops over $t \in S^{AB}_{\mathbf{a}}$ such that
  $t_{\mid_{\mathbf{a}^{\prime\prime}}} = t^{\prime\prime}$ and
  $s \in S^{AB}_{t(\mathbf{a})}$ such that $s_{\mid_{\mathbf{a}^{\prime\prime}}}
  = s^{\prime\prime}$. We write this as

  \[
    \sum_{t^{\prime\prime}, s^{\prime\prime}} \sum_{t_{\mid_{\mathbf{a}^{\prime\prime}}} = t^{\prime\prime}} z_t \sum_{s_{\mid_{t^{\prime\prime}(\mathbf{a}^{\prime\prime})}}= s^{\prime\prime}} w_s  (s\circ t)_{\mid_{\mathbf{a}^{\prime\prime}}}
  \]
  We now show that for each $t^{\prime\prime}, s^{\prime\prime}$ the
  corresponding part of the sum depends only on $t^{\prime\prime}$ and $ s^{\prime\prime}$.
  This follows from three oberservations.

  The first observation is that in the sum
  \[
      \sum_{t_{\mid_{\mathbf{a}^{\prime\prime}}} = t^{\prime\prime}} z_t \sum_{s_{\mid_{t^{\prime\prime}(\mathbf{a}^{\prime\prime})}}= s^{\prime\prime}} w_s  (s\circ t)_{\mid_{\mathbf{a}^{\prime\prime}}}
  \]
  the formal variables $(s\circ t)_{\mid_{\mathbf{a}^{\prime\prime}}}$
  are, by definition, all equal to the variable $(s^{\prime\prime}\circ t^{\prime\prime})$.
  Thus we need only consider the coefficients, given by the sum
  $$ \sum_{t_{\mid_{\mathbf{a}^{\prime\prime}}} = t^{\prime\prime}} z_t \sum_{s_{\mid_{t^{\prime\prime}(\mathbf{a}^{\prime\prime})}}= s^{\prime\prime}} w_s $$

\iffalse
  We conclude by noting three simplifications of this sum which show that for every
  $t^{\prime\prime}$ on $\mathbf{a}^{\prime\prime}$ and $s^{\prime\prime}$ on
  $t^{\prime\prime}(\mathbf{a}^{\prime\prime})$, the inner sum above is independent
  of the choice of set $\mathbf{a}$ containing $\mathbf{a}^{\prime\prime}$. \\
  The first observation is that by definition of the sums over $s$ and $t$, we
  have that the local section $(s\circ t)_{\mid_{\mathbf{a}^{\prime\prime}}}$ is
  equal to $s^{\prime\prime}\circ t^{\prime\prime}$ in every loop. Thus we need only
  consider the sum
  $$ \sum_{t_{\mid_{\mathbf{a}^{\prime\prime}}} = t^{\prime\prime}} z_t \sum_{s_{\mid_{t^{\prime\prime}(\mathbf{a}^{\prime\prime})}}= s^{\prime\prime}} w_s $$
\fi
  The second observation is that for each $t$ such that $t_{\mid_{\mathbf{a}^{\prime\prime}}} = t^{\prime\prime}$
  the sum
  $$\sum_{s_{\mid_{t^{\prime\prime}(\mathbf{a}^{\prime\prime})}}= s^{\prime\prime}} w_s$$
  is simply the $s^{\prime\prime}$ component of
  $(r^{s_0}_{t(\mathbf{a})})_{\mid_{t^{\prime\prime}(\mathbf{a}^{\prime\prime})}}$.
  As $r^{s_0}$ is a global $\mathbb{Z}$-linear section this is equal to the fixed
  parameter $w_{s^{\prime\prime}}$. So the sum in question reduces to
  $$ w_{s^{\prime\prime}} \cdot \left( \sum_{t_{\mid_{\mathbf{a}^{\prime\prime}}} = t^{\prime\prime}} z_t  \right)  $$

  The final observation, is that the remaining sum is the $t^{\prime\prime}$ component
  of $(r^{t_0}_{\mathbf{a}})_{\mid_{\mathbf{a}^{\prime\prime}}}$ which, as $r^{t_0}$
  is a global $\mathbb{Z}$-linear section, is equal to $r^{t_0}_{t^{\prime\prime}}$. This
  gives the final form of the expression for $(r^{p_0}_{\mathbf{a}})_{\mid_{\mathbf{a}^{\prime\prime}}}$
  as
  $$   \sum_{t^{\prime\prime}, s^{\prime\prime}} z_{t^{\prime\prime}}w_{s^{\prime\prime}}(t^{\prime\prime}\circ s^{\prime\prime} ) $$
  It is easy to see that the same arguments apply to $r^{p_0}_{\mathbf{a}^{\prime}}$ and
  so
  $$ (r^{p_0}_{\mathbf{a}})_{\mid_{\mathbf{a}^{\prime\prime}}} = (r^{p_0}_{\mathbf{a}^{\prime}})_{\mid_{\mathbf{a}^{\prime\prime}}}$$
  as required.
\end{proof}

In the next section, we demonstrate the power of this algorithm, using results
from Abramsky, Barbosa, Kishida, Lal and Mansfield's paper \textit{Contextuality, cohomology \& paradox}\cite{abramsky_et_al}.


==> power.tex <==
%TODO:
%-Theorem 1: You need to explain what you mean by "a finite Ring
%represented as a relational structure [...] over sigma".  Perhaps a
%formal definition should come earlier in the paper.
%
%-Observation 1: You state it for "any CSP(A,B)" but a measurement
%scenario <X.M,R> has only been defined for the case where R is a
%ring.  Do you mean to generalize the notion of measurement scenario?
%Or restrict the observation to the case where B is a ring?
%
%
%

In this section, we demonstrate the power of the cohomological $k$-consistency
algorithm by proving that it can decide the solvability of systems of equations
over finite fields.

To express the main theorem of this section in terms of the finite relational structures
on which our algorithm is defined, we first need to fix a notion of a finite ring represented
as a relational structure. Let $R$ be a finite ring. Define $\sigma_R$
as the (countable) set of relational symbols $\{ E^m_{\mathbf{a},b} \ \mid \ m \in \mathbb{N}, \mathbf{a} \in R^{m}, b \in R \}$ where the arity for each $E^m_{\mathbf{a},b}$ is $m$. For any
finite $\sigma \subset \sigma_R$ the \emph{representation of $R$ as a relational
structure over $\sigma$} is the structure with universe the elements of $R$
and for each symbol $E^m_{\mathbf{a},b} \in \sigma$ the related tuples are those
$(r_1, \ldots , r_m) \in R^m$ such that
$$ a_1 \cdot r_1 + \dots a_m \cdot r_m = b $$
When $R$ is represented in this way as a relational structure over $\sigma$, then
any instance of the constraint satisfaction problem $\mathbf{CSP}(R)$ specifies
a system of $R$-linear equations where each of the equations takes is of the form
$$ a_1 \cdot x_1 + \dots a_m \cdot x_m = b $$
for some $E^m_{\mathbf{a},b}\in \sigma$.

With this notation established we can state the theorem we prove in this section.

\begin{theor} \label{thm:rings}
  For any finite ring $R$ represented as a relational structure over a finite signature $\sigma \subset \sigma_R$,
  there is a $k$ such that the cohomological $k$-consistency algorithm decides $\mathbf{CSP}(R)$.\\
  Alternatively stated, there exists a $k$ such that for all $\sigma$-stuctures $A$
  $$ A \rightarrow^{\mathbb{Z}}_{k} R \iff A \rightarrow R  $$
\end{theor}

This theorem is notable because for such rings $R$
there are families of structures $A_k$ such that $A_k \rightarrow_k R$ but $A_k \not \rightarrow R$, see
\cite{federvardi}.
Furthemore there exist pairs $(A_k, B_k)$ where $A_k \equiv_k B_k$, $B_k \rightarrow R$ and
$A_k \rightarrow_k R$ but $A_k \not \rightarrow R$, see \cite{AtseriasBulatovDawar}.
As the sequence of relations $\equiv_k$ bounds
the expressive power of FPC, this effectively proves
the solvability of systems of linear equations over $\mathbb{Z}$ is not expressible in FPC, a result
which was until now unknown to the author.\\

To prove this theorem we invoke a result from \cite{abramsky_et_al}
which considers a similar set-up to that seen in the previous sections and proves
a result relating the non-existence of solutions to a system of linear equations over
a ring $R$ to the non-triviality of a family of cohomological ``obstructions''.
We will recall their set-up, the relevant result and a characterisation of these
cohomological ``obstructions'' in terms of global $\mathbb{Z}$-linear sections before
proving Theorem \ref{thm:rings}.

\subsection{Result from \textit{Contextuality, cohomology \& paradox}}

In order to state the relevant theorem, we start with some preliminary definitions.
Let a \emph{ring-valued measurement scenario} be a triple $\langle X, \mathcal{M}, R \rangle$
where $X$ is a finite set, $\mathcal{M}$ is a downward closed cover of $X$ and $R$ is a ring.
An \emph{$R$-linear equation} on $\langle X, \mathcal{M}, R \rangle$ is a triple
$\phi = (V_{\phi}, a, b)$ where $V_{\phi} \in \mathcal{M}$, $a: V_{\phi}\rightarrow R$
and $b \in R$. Then for any $s \in R^{V_{\phi}}$ we say that $s \models \phi$ if
$$ \sum_{m \in V_{\phi}} a(m)s(m) = b   $$
 in the ring $R$. \\

An \emph{empirical model} $S$ on $\langle X, \mathcal{M}, R \rangle$ is a collection
of sets $\{ S_C \}_{C \in \mathcal{M}}$ where for each $C$, $S_C \subset R^C$ satisfying
the following compatibility condition for all $C, C' \in \mathcal{M}$
$$ \{s_{\mid_{C\cap C'}} \ \mid \ s \in S_C \} = \{s'_{\mid_{C\cap C'}} \ \mid \ s' \in S_{C'} \}  $$
We make the following observation linking relational structures over signatures
$\sigma \subset \sigma_R$ and empirical models which will be useful later.
\begin{obs}\label{obs:emp_model}
For any $\mathbf{CSP}(A,R)$ and $S \subset \mathbf{Hom}_k(A,R)$ which is non-empty,
and downward-closed and satisfies the forth property
 then the local sections of $S$ form an
empirical model for the measurement scenario $\langle A, A^{\leq k}, R \rangle$.
\end{obs}

For an empirical model $S$ on an $R$-valued measurement scenario, the \emph{$R$-linear theory}
of $S$ is the set of $R$-linear equations
$$ \mathbb{T}_R(S) = \{ \phi \ \mid \ \forall s \in S_{V_{\phi}}, \ s \models \phi \} $$

If $\mathbb{T}_R(S)$ is inconsistent (i.e.\ there is no $R$-assignment to all the
variables in $X$ simultaneously satisfying each of the $R$-linear equations in
the theory), then the empirical model $S$ is said to be
``all-vs-nothing for $R$'', written $\mathbf{AvN}_{R}(S)$.

We can now state the following results that we need for Theorem \ref{thm:rings}. The first result shows an important implication about the
cohomological obstructions in an empirical model which has an inconsistent $R$-linear theory.
\begin{theor}[Abramsky, Barbosa, Kishida, Lal, Mansfield \cite{abramsky_et_al}]\label{thm:avn}
For any ring $R$ and any $R$-valued measurement scenario $\langle X, \mathcal{M}, R \rangle$
and any empirical model $S$ we have that
$$ \mathbf{AvN}_{R}(S) \implies \mathbf{CSC}_{\mathbb{Z}}(S)$$
where $\mathbf{CSC}_{\mathbb{Z}}(S)$ means that for every local section $s$ in $S$ the
``cohomological obstruction'' of Abramsky, Barbosa and Mansfield $\gamma(s)$ is
non-zero.
\end{theor}

Next we have a result due to Abramsky, Barbosa and Mansfield which establishes
this useful equivalent condition for $\mathbf{CSC}_{\mathbb{Z}}(S)$
\begin{theor}[Abramsky, Barbosa, Mansfield \cite{ab_man_barb}] \label{thm:Z_ext}
  For any empirical model $S$, $\mathbf{CSC}_{\mathbb{Z}}(S)$ if and only if
  for every $s \in S_C$ there is no collection $\{r_{C'} \in \mathbb{Z}S_{C'} \}_{C' \in \mathcal{M}}$
  such that $r_C = s$ and for all $C_1, C_2 \in \mathcal{M}$
  $$ r_{C_1 \mid_{C_1 \cap C_2}} = r_{C_2 \mid_{C_1 \cap C_2}} $$
\end{theor}

This condition is precisely what inspired the cohomological $k$-consistency algorithm
and in the next section we show how these two results imply Theorem \ref{thm:rings}.

\subsection{Proof of Theorem \ref{thm:rings}}
We now prove the main theorem of this section.

\begingroup
\def\thelem{\ref{thm:rings}}
\begin{theor}
For any finite ring $R$ represented as a relational structure over a finite signature $\sigma$,
there is a $k$ such that the cohomological $k$-consistency algorithm decides $\mathbf{CSP}(B)$.\\
Alternatively, there exists a $k$ such that for all $\sigma$-stuctures $A$
$$ A \rightarrow^{\mathbb{Z}}_{k} R \iff A \rightarrow R  $$
\end{theor}
\addtocounter{lem}{-1}
\endgroup

\begin{proof}
The direction $A \rightarrow R \implies A \rightarrow^{\mathbb{Z}}_k R$ is easy
and is true for all signatures $\sigma$ and all $k\leq |A|$. Indeed note that to any
homomorphism $f : A \rightarrow R$ we can associate the  set $S_f = \{f_{\mid_{\mathbf{a}}} \}_{\mathbf{a}\in A^{\leq k}} \subset \mathbf{Hom}_k(A,B)$. It is not hard to see that $S_f$ is downward closed, has the forth
property and that $S_f$ is itself a global section witnessing the $\mathbb{Z}$-extendability
of each $f_{\mid_{\mathbf{a}}} \in S_f$. By Observation \ref{obs:consist_set}, this
implies that $A \rightarrow^{\mathbb{Z}}_{k} R$. \\

This leaves the more challenging direction, that there exists a $k$ such that
$A \not\rightarrow R \implies A \not\rightarrow^{\mathbb{Z}}_k R$ for all $A$. Suppose
that the maximum arity of a relation in $\sigma$ is $n$. Then as $R$ is a relational
model of a finite ring we know that each relation on $R$ is of the form
$E^{m}_{\mathbf{a}, b} = \{ (r_1, \ldots , r_m) \ \mid \ \sum_{i} a_i\cdot r_i = b \}$
where $\mathbf{a}$ is an $m$-tuple of elements of the ring $R$ and $b$ is an element
of $R$. We show that $k = n$ will suffice to identify all unsatisfiable instances $A$.

For $R$ and $\sigma$ as above any instance $\mathbf{CSP}(A,R)$ is specified by a set $A$
of variables where each related tuple $(x_1, \ldots , x_m ) \in (E^m_{\mathbf{a}, b})^A$
specifies an $R$-linear equation $\sum_{i} a_i\cdot x_i = b$. Call the collection
of such equations $\mathbb{T}^A$.
The fact that there is no homomorphism $A \rightarrow R$ is exactly the statement that $\mathbb{T}^A$
is unsatisfiable. Taking $k = n$, we have that the $R$-linear theory
 $\mathbb{T}_R(\mathbf{Hom}_k(A,R))$ (as defined in the previous section) contains
 $\mathbb{T}^A$ and so is unsatisfiable. We now show how this is sufficient to prove the theorem.

Consider running the cohomological $k$-consistency algorithm on the pair $(A, R)$
we get $S_0 = \overline{\mathbf{Hom}_k(A, R)}$. If $S_0 = \emptyset$ we are done.
Otherwise, by Observation \ref{obs:emp_model}, $S_0$ can be considered as an empirical
model on the measurement scenario $\langle A, A^{\leq k}, R \rangle$. Furthemore,
as $S_0 \subset \mathbf{Hom}_k(A, R)$, we have that $\mathbb{T}_R(S_0) \supset \mathbb{T}_R(\mathbf{Hom}_k(A,R))$.
This means in particular that $\mathbb{T}_R(S_0)$ is unsatisfiable by the assumption
that $A \not\rightarrow R$. By Theorems \ref{thm:avn} and \ref{thm:Z_ext}, this
means that no local section $s$ of $S_0$ is $\mathbb{Z}$-extendable in $S_0$, so
$S_1 = \emptyset$. So the cohomological $k$-consistency algorithm
rejects $(A, R)$ and $A \not\rightarrow^{\mathbb{Z}}_k R$, as required.


\end{proof}

It is notable that in the proof of this theorem, we see that the cohomological $k$-consistency
algorithm decides unsatisfiability of these systems of equations after just one iteration of its loop.
A future version of this work will investigate whether multiple iterations are required in
over different CSP domains. For now, we retain the iterative nature of the algorithm to
guarantee the conclusion in Observation \ref{obs:consist_set}.

It is known, from a result of Atserias, Bulatov and Dawar\cite{AtseriasBulatovDawar},
that the solvability of systems of linear equations over finite rings
(even in a fixed number of variables per equation) is not definable in FPC . As
the cohomological $k$-consistency consistency algorithm can decide the solvability of these systems of equations
by Theorem \ref{thm:rings} by repeatedly checking solvability of systems of linear equations
over $\mathbb{Z}$, we have the following important corollary of Theorem \ref{thm:rings}.

\begin{cor}\label{cor:fpc}
  The solvability of systems of linear equations over $\mathbb{Z}$ is not expressible in FPC.
\end{cor}

In the next section, we introduce an efficient algorithm approximating structure isomorphism
which, similar to the cohomological $k$-consistency algorithm, is based on checking solvability
systems of linear equations over $\mathbb{Z}$. We will show that this algorithm
can distinguish structures which differ on other properties which are known to
be inexpressible in FPC.



\iffalse
We would like to use this result to show that adding the ability to solve $\mathbb{Z}$-linear
equations to FPC is enough to distinguish all known examples of structures which
are decidably non-isomorphic in \texttt{PTIME} but whose non-isomorphism is not
captured by FPC. For that we use these methods to construct an equivalence of
relational structures in the next section.
\fi

